VoronoiNet: General Functional Approximators with Local Support

Voronoi diagrams are highly compact representations that are used in various Graphics applications. In this work, we show how to embed a differentiable version of it -- via a novel deep architecture -- into a generative deep network. By doing so, we achieve a highly compact latent embedding that is able to provide much more detailed reconstructions, both in 2D and 3D, for various shapes. In this tech report, we introduce our representation and present a set of preliminary results comparing it with recently proposed implicit occupancy networks.

==> 2_related.tex <==
\section{Related work}
\label{sec:related}

\begin{itemize}
    \item The optimization version of our problem \cite{voroapprox}
    \item Modify grids into voro make them conformal to signal \cite{vorogrids}
    \item Fast centroidal voronoi optimization \cite{voroopt}
\end{itemize}

\lorem{1}

==> OLD.tex <==






==> fig/onecol.tex <==
\begin{figure}
\centering
\begin{overpic} 
[width=\linewidth]
{fig/onecol.pdf}
\end{overpic}
\caption{
One column template
}
\label{fig:onecol}
\end{figure}

==> fig/twocol.tex <==
\begin{figure*}[ht]
\centering
\begin{overpic} 
[width=\linewidth]
{fig/twocol.pdf}
\end{overpic}
\caption{
Two column template
}
\label{fig:twocol}
\end{figure*}

